Towards Full-Fledged Argument Search: A Framework for Extracting and Clustering Arguments from Unstructured Text

Argument search aims at identifying arguments in natural language texts. In the past, this task has been addressed by a combination of keyword search and argument identification on the sentence- or document-level. However, existing frameworks often address only specific components of argument search and do not address the following aspects: (1) argument-query matching: identifying arguments that frame the topic slightly differently than the actual search query; (2) argument identification: identifying arguments that consist of multiple sentences; (3) argument clustering: selecting retrieved arguments by topical aspects. In this paper, we propose a framework for addressing these shortcomings. We suggest (1) to combine the keyword search with precomputed topic clusters for argument-query matching, (2) to apply a novel approach based on sentence-level sequence-labeling for argument identification, and (3) to present aggregated arguments to users based on topic-aware argument clustering. Our experiments on several real-world debate data sets demonstrate that density-based clustering algorithms, such as HDBSCAN, are particularly suitable for argument-query matching. With our sentence-level, BiLSTM-based sequence-labeling approach we achieve a macro F1 score of 0.71. Finally, evaluating our argument clustering method indicates that a fine-grained clustering of arguments by subtopics remains challenging but is worthwhile to be explored.

==> sections/results2.tex <==


\begin{table*}[tb]
\centering
\caption{Results of argument identification on the \emph{Student Essay} data set.
%Precision ($P$) and recall ($R$) are reported separately for the classes $B$ (sentences starting an argument), $I$ (sentences continuing an argument) and $O$ (sentences not belonging to any argument). In addition to the macro $F_1$-score and the weighted $F_1$-score, we report the macro $F_1$-score $F_{1, macro}^{B, I}$ computed only for the classes $B$ and $I$.
}
\label{tab:Results:Segmentation}
\begin{small}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}l cc cc cc ccc@{}}
\toprule
& \multicolumn{2}{c}{\emph{B}}& \multicolumn{2}{c}{\emph{I}}& \multicolumn{2}{c}{\emph{O}}& \multicolumn{2}{r}{}\\ \cline{2-3} \cline{4-5} \cline{6-7}

 & $Prec.$ & $Rec.$  
 & $Prec.$ & $Rec.$  
 & $Prec.$ & $Rec.$  
 &$F_{1, macro}$ & $F_{1, weighted}$ &$F_{1, macro}^{B, I}$ \\
\midrule
majority class 
& 0.000 & 0.000
& 0.719 & 1.000 
& 0.000 & 0.000 
&	0.279 & 0.602 & 0.419\\
$FNN_{avg}^{bert}$  
& 0.535 & 0.513 
& 0.820 & 0.836	
& 0.200 & 0.160 
& 0.510 & 0.736 & 0.675\\
$FNN_{cls}^{bert}$  
& 0.705 & 0.593	
& 0.849 & 0.916	
& \textbf{0.400} & 0.080 
& 0.553 & 0.805 & 0.763\\
$BILSTM_{avg}^{bert}$  
& 0.766 & 0.713 
& 0.885 & 0.930 
& 0.000 & 0.000 
& 0.549 & 0.846 & 0.823 \\
$BILSTM_{cls}^{bert}$  
 & \textbf{0.959}  & \textbf{0.914}
 & \textbf{0.967}  & \textbf{0.985}
 & 0.208 & \textbf{0.200}
& \textbf{0.705} & \textbf{ 0.951} & \textbf{0.956} \\
\bottomrule
\end{tabular}
}
\end{small}
\end{table*}


\begin{table*}[tb]
\centering 
\caption{Results of argument identification on the \emph{debate.org} data set; model trained on \emph{Student Essay} and \emph{debate.org}.
%The first row displays the result for the BiLSTM being pretrained on the \emph{Student Essay} data set and directly applied on the \emph{debate.org} data set relative to training it from scratch on the \emph{debate.org} dataset as shown in the second row.
}
\label{tab:Results:SegORG}
\begin{small}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}ll cc cc cc cc@{}}
\toprule
& & \multicolumn{2}{c}{\emph{B}}& \multicolumn{2}{c}{\emph{I}}& \multicolumn{2}{c}{\emph{O}}& \multicolumn{2}{r}{}\\ 
\cline{3-8}
&\emph{trained on}
 & $Prec.$ & $Rec.$  
 & $Prec.$ & $Rec.$  
 & $Prec.$ & $Rec.$  
 &$F_{1, macro}$ & $F_{1, weighted}$ \\
\midrule
$BILSTM_{cls}^{bert}$ & \emph{essay}
& 0.192 & 0.312 
& 0.640 & 0.904 
& 1.000 & 0.015 
& 0.339 & 0.468\\
$BILSTM_{cls}^{bert}$  &\emph{debate.org}
& 1.000 & 0.021 
& 0.646 & 0.540 
& 0.381 & 0.640 
& 0.368 & 0.492\\
\bottomrule
\end{tabular}
}
\end{small}
\end{table*}


\subsection{Evaluation Results} %  and Discussion}
\label{sec:Results}

In the following, we present the evaluation results for the tasks topic clustering, argument identification, and argument clustering.
%We use the evaluation metrics 
% described in Section \ref{sec:Background}. 
%precision, recall and $F_1$-measure concerning the classification, and Adjusted Rand Index (ARI), homogeneity, and BCubed $F_1$-score concerning the clustering. 
%









\begin{table*}[h]
\centering
\caption{Results of the clustering of arguments of the \emph{debatepedia} data set by topical aspects. \emph{across topics}:~tf-idf scores are computed across topics, \emph{without noise}:~{HDBSCAN} is only evaluated on those examples which are not classified as noise.}
% $Ho$:~Homogeneity, $Co$:~Completeness, $F_1$:~BCubed~$F_1$-score, \emph{across topics}:~tf-idf scores are computed across topics, \emph{without noise}:~{HDBSCAN} is only evaluated on those examples which are not classified as noise.}
\label{tab:Results:ASUnsupervised}
\begin{small}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}l l l cccc l@{}}
\toprule
 Embedding & Algorithm & Dim. Reduction & $ARI$ & $Ho$	&$Co$	& $BCubed~F_1$ & Remark\\
\midrule
tf-idf 		& HDBSCAN 	& UMAP 	& 0.076 & 0.343	&0.366& 0.390 & \\
tf-idf 		& HDBSCAN 	& UMAP 	& 0.015 & 0.285	&0.300& 0.341 &\emph{across topics} \\
tf-idf 		& HDBSCAN 	& $-$ 	& \textbf{0.085} & \textbf{0.371}	&\textbf{0.409}& \textbf{0.407}	& \\
tf-idf 		& k-means 	& $-$ 	& 0.058 & 0.335	&0.362& 0.397 & \\
tf-idf 		& k-means 	& $-$ 	& 0.049 & 0.314	&0.352& 0.402 &\emph{across topics} \\
\midrule
bert-cls 	& HDBSCAN 	& UMAP 	& 0.030	& 0.280	&0.298& 0.357 & \\
bert-cls 	& HDBSCAN 	& $-$		& 0.016	& 0.201	&0.324& 0.378 & \\
bert-cls 	& k-means 	& $-$		& 0.044	& 0.332	&0.326& 0.369 & \\
\midrule
bert-avg 	& HDBSCAN 	& UMAP 	& 0.069	& 0.321	&0.352& 0.389 & \\
bert-avg 	& HDBSCAN 	& $-$		& 0.018	& 0.170	&0.325& 0.381 & \\
bert-avg 	& k-means 	& $-$		& 0.065	& 0.337	&0.349& 0.399 & \\
\midrule
tf-idf 		& HDBSCAN 	& $-$ 	& 0.140 & 0.429	&0.451& 0.439	&\emph{without noise}\\
\bottomrule
\end{tabular}
}
\end{small}
\end{table*}





\begin{figure*}[h]
\centering
\includegraphics[width = 0.42\textwidth]{key_results/AS/hdbscan_scatterplot2}
\includegraphics[width = 0.42\textwidth]{key_results/AS/kmeans-bert_scatterplot2}
\caption{Argument clustering results (measured by $ARI$, $BCubed F_1$, and $homogeneity$) for HDBSCAN on tf-idf embeddings and k-means on  \emph{bert-avg} embeddings.}
%with respect to the number of arguments per topic.}
\label{fig:Results:Scatterplot}
\end{figure*}







% \subsection{Main Findings}

\textbf{Topic Clustering.} 
We evaluate unsupervised topic clustering based on the 170 topics from the \textit{debatepedia} data set. Given Table~\ref{tab:Results:ClusteringUnsupervised}, we see that density-based clustering algorithms, such as {HDBSCAN}, applied to tf-idf document embeddings are particularly suitable for this task and clearly outperform alternative clustering approaches. We find that their ability to handle unclear examples as well as clusters of varying shapes, sizes, and densities is crucial to their performance. 
% Disregarding the 4\% of documents not being assigned to any topic cluster, 
{HDBSCAN} in combination with a preceding dimensionality reduction step achieves an $ARI$ score of 0.779. However, these quantitative results must be considered from the standpoint that topics in the \emph{debatepedia} data set are overlapping and, thus, the reported scores are lower bound estimates.
%We illustrate this for the case of the topics \emph{`Gay adoption'} and \emph{`Gay marriage'}.
% 
%Based on a qualitative assessment of the clustering results for \emph{debatepedia} data set, 
When evaluating the clustering results for the \emph{debatepedia} data set qualitatively, 
we find that many predicted clustering decisions are reasonable but evaluated as erroneous in the quantitative assessment. For instance, 
we see that 
documents on \textit{gay parenting} 
appearing in the debate about \textit{gay marriage} can be assigned to a cluster with documents on \textit{gay adoption}.
%In the quantitative evaluation based on the topics determined by \emph{debatepedia} data set, however, this and similar clustering decisions are often assessed as incorrect.

Furthermore, we investigate the impact on the recall of relevant documents and observe a clear improvement of topic clusters over keyword matching for argument-query matching. % We illustrate this based on an exemplary search query about \emph{gay adoption}. 
For instance, given the topic \emph{gay adoption}, many documents from debatepedia.org use related terms like \emph{homosexual} and \emph{parenting} instead of explicitly mentioning \emph{`gay'} and \emph{`adoption'} and, thus, cannot be found by a keyword search.

%%removed 2-step approach
%As an alternative to the unsupervised topic clustering, we investigate whether a two-step approach consisting of computing pairwise similarities followed by an agglomerative clustering step on the derived distance matrix achieves even better results. Despite its good performance, this two-step approach does not outperform our results from the fully unsupervised setting.
We additionally evaluate the inductive capability of our topic clustering approach by applying them to debates from debate.org (see Table~\ref{tab:Results:ClusteringUnsupervisedORG}). We observe that the application of the unsupervised clustering on  tf-idf embeddings for debates from debate.org achieves a solid mediocre $ARI$ score of 0.436.

%SEG
\textbf{Argument Identification.} 
To evaluate the identification of argumentative units based on sentence-level sequence-labeling, we apply our approach to the \emph{Student Essay} data set (see Table~\ref{tab:Results:Segmentation}) and achieve a macro $F_1$ score of 0.705 with a BiLSTM-based sequence-learning model on sentence embeddings computed with BERT. Furthermore, we observe a strong influence of the data sources on the results for argument identification. For instance, in the case of the \textit{Student Essay} data set,  information about the current sentence as well as the surrounding sentences is available yielding accurate segmentation results ($F_{1,macro}=0.71$, $F_{1,macro}^{BI}=0.96$).

%AS
\textbf{Argument Clustering.}
Finally, we proposed an approach to cluster arguments consisting of one or several sentences by topical aspects. We evaluate the clustering 
% results 
based on tf-idf and BERT embeddings of the arguments (see Table~\ref{tab:Results:ASUnsupervised}). Overall, the performance of the 
% all 
investigated argument clustering methods is considerably low. We find that this is due to the fact that information on topical aspects is scarce and often underweighted in case of multiple sentences. 
% As Figure~\ref{fig:Results:Scatterplot} showing the performance of the two models with respect to the number of arguments in each topic, 
Given Figure~\ref{fig:Results:Scatterplot}, we can observe that the performance of the clustering does not depend on the number of arguments.




%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
%


\if0 



\begin{table}
\centering
\caption{Confusion matrices of $BILSTM_{cls}^{bert}$: Rows represent ground-truth labels and columns represent predictions.\\Left: \emph{Student Essay} data set, Right: \emph{debate.org} data set.}
\label{tab:Results:CM}
\begin{small}
\begin{tabular}{c| ccc}
& B & I & O\\
\midrule
B&15 	& 33 	& 0\\
I&24	& 226	& 0 \\
O&39 	& 94 	& 2\\
\bottomrule
\end{tabular}
\hspace{1cm}
\begin{tabular}{c| ccc}
& B & I & O\\
\midrule
B&1 	& 24 & 23\\
I&0	& 135 & 115 \\
O&0 	& 50 	& 85\\
\bottomrule
\end{tabular}
\end{small}
\end{table}




\begin{table*}[tb]
\centering
\caption{Overview of the topics with the highest $ARI$ scores for HDBSCAN and k-means.}
%and evaluated on all non-noise examples (\emph{top}) and k-means based on \emph{bert-avg} (\emph{bottom}) are the six topics that resulted in the . \\
%$n_{true}$:~Number of ground-truth clusters, $n_{pred}$:~Number of predicted clusters,}
\label{tab:Results:BestTopics}
\begin{small}
\begin{tabular}{@{}l p{7cm} rr cccc @{}}
\toprule
&Topic & \#$Clust._{true}$ & \#$Clust._{pred}$ & $ARI$ & $Ho$	&$Co$	& $BCubed~F_1$  \\
\toprule
\multicolumn{8}{c}{\textbf{HDBSCAN based on tf-idf embeddings}}\\
\midrule
1 &Rehabilitation vs retribution
&2 &3 & 0.442 &1.000 &0.544 &0.793 \\
2 &Manned mission to Mars
&5 &6 &0.330 & 0.461&0.444 & 0.515\\
3 & New START Treaty
&5 &4 &0.265 &0.380 &0.483 &0.518 \\
4 &Obama executive order to raise the debt ceiling
&3 &6 & 0.247 &0.799 &0.443 &0.568 \\
5 &Republika Srpska secession from Bosnia and Herzegovina
&4 &6 &0.231 &0.629 &0.472 &0.534 \\
6& Ending US sanctions on Cuba
&11 &9 & 0.230&0.458 &0.480 &0.450 \\
\toprule
\multicolumn{8}{c}{\textbf{k-means based on \emph{bert-avg} embeddings}}\\
\midrule

1 &Bush economic stimulus plan
&7 &5 & 0.454 &0.640 &0.694 &0.697 \\
2 &Hydroelectric dams
&11 &10 &0.386 & 0.570&0.618 & 0.537\\
3 & Full-body scanners at airports
&5 &6 &0.301 &0.570 &0.543 &0.584 \\
4 &Gene patents
&4 &7 & 0.277 &0.474 &0.366 &0.476 \\
5 &Israeli settlements
&3 &4 &0.274 &0.408 &0.401 &0.609 \\
6& Keystone XL US-Canada oil pipeline
&2 &3 & 0.269&0.667 &0.348 &0.693 \\
\bottomrule
\end{tabular}
\end{small}
\end{table*}


%Krippendorff' $\alpha$ of 0.47 
\begin{figure}[tb]
\centering
\includegraphics[width=0.4\textwidth]{key_results/AS/ARI_two_models3}
\includegraphics[width=0.4\textwidth]{key_results/AS/ARI_hdbscan2}
\caption{Argument clustering consensus based on the $ARI$ between (top) HDBSCAN and k-means  score and (bottom) HDBSCAN model and the ground-truth.}
\label{fig:Results:Hist}
\end{figure}



\begin{figure}[tb]
\centering
\includegraphics[width=0.7\linewidth]{images/subtopic_argument_correlation2}
\caption{Linear regression of arguments and their topical aspects for the \emph{debatepedia} data set.}%The number of topical aspects is given by the number of subtopics for each topic in the \emph{debatepedia} data set and the linear regression and its equation are displayed.}
%\caption{Scatterplot of the number of arguments and the number of  topical aspects per topic for the \emph{debatepedia} dataset. The number of topical aspects is given by the number of subtopics for each topic in the \emph{debatepedia} data set and the linear regression and its equation are displayed.}
\label{fig:Results:Correlation}
\end{figure}


\subsubsection{Topic Clustering}
\label{sec:Results:DS}
The results of  the unsupervised clustering approach are shown in Table \ref{tab:Results:ClusteringUnsupervised}, based
% introduced in section~\ref{sec:Approach} 
on a subset of the \emph{debatepedia} data set with 170 topics. The simple model $ARGMAX_{none}^{tfidf}$ computes clusters based on words with the highest tf-idf score within a document. Its $ARI$ score of $0.470$ indicates that many topics in the \emph{debatepedia} data set can already be represented by a single word. Considering the $ARGMAX_{lsa}^{tfidf}$ model, the lower $ARI$ score of $0.368$ indicate that using the topics found by LSA does not add value compared to tf-idf vectors. 
%Similarly, the performance of $ARGMAX_{lsa}^{tfidf}$ indicates how well the topics inherent in the LSA vectors, represented by a distribution over terms, match the ground-truth topics. However, the $ARI$-score of $0.368$ indicates that using the topics found by LSA does not bring an additional value over using plain tf-idf vectors for this dataset. 

Furthermore, we evaluate k-means with the density-based clustering algorithm HDBSCAN. 
First, we find that $HDBSCAN_{lsa + umap}^{tfidf}$ and  $KMEANS_{none}^{tfidf}$  with $ARI$ scores of $0.694$ and $0.703$, respectively, achieve a comparable performance on the tf-idf vectors. However, since HDBSCAN accounts for noise is the data which it pools within a single cluster, the five rightmost columns of Table \ref{tab:Results:ClusteringUnsupervised} have to be considered when deciding on a clustering method for further use. When excluding the noise cluster from the evaluation and thereby considering only approx. 96\% of instances where $HDBSCAN_{lsa + umap}^{tfidf}$ and $HDBSCAN_{umap}^{tfidf}$ are sure about the cluster membership, the $ARI$ score of the clustering amounts to $0.78$. Considering that 21.1\% of $HDBSCAN_{none}^{tfidf}$ are classified as noise, compared to the 4.3 \% of $HDBSCAN_{umap}^{tfidf}$, we conclude that applying an UMAP dimensionality reduction step before the HDBSCAN clustering is essential for its performance on the \emph{debatepedia} data set. 
%Since the quality of the resulting clusters from the topic clustering step influences the results of the argument clustering step, clustering

\textbf{Qualitative Evaluation.} Looking at the predicted clusters reveals that many of the clusters considered as erroneous are reasonable. For example, $HDBSCAN_{lsa + umap}^{tfidf}$ maps the document with the title \emph{`Military recruiting: Does NCLB rightly allow military recruiting in schools?'} of the topic \emph{`No Child Left Behind Act'} to the cluster representing the topic \emph{`Military recruiting in public schools'}. 
Another such example is a cluster that is largely comprised of documents about \emph{`Gay adoption'}, but contains one additional document \emph{`Parenting: Can homosexuals do a good job of parenting?'} from the topic \emph{`Gay marriage'}.
%When evaluating the clusters, these two decisions should not be considered as mistakes. 



% subsubsubsection*
%\textbf{Model transferability.}
\textbf{Inductive Generalization.}
We apply the unsupervised approach to the \emph{debate.org} data set to evaluate whether the model is able to generalize. The results, given in Table \ref{tab:Results:ClusteringUnsupervisedORG}, show that the unsupervised approach using  HDBSCAN and k-means leads to far better results with $ARI$ scores of 0.354 and 0.436, respectively. K-means performs on the \emph{debate.org} data set distinctly better than HDBSCAN because the \emph{debate.org} data set is characterized by an high number of single-element topics. In contrast to k-means, HDBSCAN does not allow single-element clusters, thus getting pooled into a single noise cluster. Furthermore, this is reflected by the different numbers of clusters as well as the lower homogeneity scores of HDBSCAN of 0.633 and 0.689 compared to 0.822 of k-means while having a comparable completeness of approx. 0.8.

% subsubsubsection*
\textbf{Topic Clusters for Argument-Query Matching.}
Applying a keyword search would retrieve only a subset of the relevant arguments that mention the search phrase explicitly. Combining a keyword search on documents with the clusters found by $HDBSCAN$, enables an argument search framework to retrieve arguments from a broader set of documents. For example, in the data set \textit{debatepedia.org}, we observe that clusters of arguments related to \emph{gay adoption} include words like \emph{parents}, \emph{mother}, \emph{father},  \emph{sexuality}, \emph{heterosexual}, and \emph{homosexual} while neither \emph{gay} nor \emph{adoption} are not mentioned explicitly.
%
%Not found by keyword search but in the same cluster
%\begin{itemize}
%\item \textbf{Natural: Is being brought up by a same sex couple natural?} \emph{Children do not need distinct male and female parental role-models. What children need first is love, compassion, and care from their parents. In addition, children are highly influenced by their social environment as much as their parents, making it unreasonable to place such a high importance on the attributes that parents display.}
%\item \textbf{Gay influence: Do gay parents influence children to become homosexual?} \emph{A child's primary role models are his or her parents.} \emph{Bringing a heterosexual child up in a gay household gives them a distorted view of a minority sexuality, just as a girl brought up by two men would fail to benefit from a feminine influence.}
%\item \textbf{Quality: Are homosexual parents of equal quality in raising children?} \emph{Numerous studies indicate that homosexual parenting has proven equally capable as heterosexual parenting.}
%\end{itemize}
%
%Applying a keyword search for \emph{`gay adoption'} by retrieving only the single arguments which mention \emph{gay} and \emph{adoption} explicitly would miss a substantial portion of the relevant arguments in this dataset. In contrast, combining a keyword search on documents with the clusters found by $HDBSCAN_{umap}^{tfidf}$ by considering all documents which appear together in a cluster with those documents mentioning \emph{gay} and \emph{adoption} explicitly, would match all arguments from the topic \emph{`Gay adoption'} plus an additional one about gay parenting from the \emph{`Gay marriage'} topic.
%
%***************************SEGMENTATION*************************************

\subsubsection{Argument Identification}
\label{sec:Results:SEG}


%We analyze the results of the argument segmentation on the \emph{Student Essay} and \emph{debate.org} data sets. 

The results of the argument identification step based on the \emph{Student Essay} data set is given in Table \ref{tab:Results:Segmentation}. We evaluate a BiLSTM model in a sequence-labeling setting compared to a feedforward neural network (FNN) in a classification setting in order to investigate the importance of context for the identification of arguments. Using the BiLSTM improves the macro $F_1$ score relative to the feedforward neural network on the \emph{bert-avg} embeddings by 3.9\% and on the \emph{bert-cls} embeddings by 15.2\%. Furtheremore, we evaluate the effects of using the sentence embedding \emph{bert-avg} and \emph{bert-cls}. 
%\emph{bert-avg} which is computed by  averaging BERT word embeddings and the sentence embedding \emph{bert-cls} which is the output of BERT corresponding to the $[CLS]$ token.
Using \emph{bert-cls} embeddings increases the macro $F_1$ score by 4.3\% in the classification setting and by 15.6\% in the sequence-learning setting relative to using \emph{bert-avg}. Considering also the sequence-learning and classification results, we conclude that the \emph{bert-cls} embeddings encode important additional information which gets only utilized in a sequence-learning setting.

Our results also reflect the peculiarity of the \emph{Student Essay}'s training data set that most sentences are part of an argument and only $\sim$3\% of the sentences are labeled as outside (`O'). Accordingly, the models observe hardly any examples for outside sentences during training and, thus, have difficulties in learning to distinguish them from other sentences. Overall, this is reflected by the very low precision and recall for the class `O'. Considering the fact that the correct identification of a `B' sentence alone is already enough to separate two arguments from each other, the purpose of labeling a sentence as `O' is restricted to classifying the respective sentence as non-argumentative. Therefore, in case of the \emph{Student Essay} data set, the task of separating two arguments from each other becomes much more important than separating non-argumentative sentences from arguments. Therefore, the last column of Table \ref{tab:Results:Segmentation} indicates the macro $F_1$ score only for the `B' and `I' labels with a macro $F_1$ score of 0.956 for our best model. This reflects the model's high ability to separate arguments from each other.


%The first row displays the result for the BiLSTM being pretrained on the \emph{Student Essay} data set and directly applied on the \emph{debate.org} data set relative to training it from scratch on the \emph{debate.org} dataset as shown in the second row.

Furthermore, we evaluate whether the previously best-performing model $BILSTM_{cls}^{bert}$ is able to identify arguments on the \emph{debate.org} data set if trained on the \emph{Student Essay} data set. The results are given in Table \ref{tab:Results:SegORG}.
%the \emph{essay} data set pretrained $BILSTM_{cls}^{bert}$ model directly to the \emph{debate.org} data set. 
The pretrained model performs very poor on \emph{`O'} sentences since not many examples of \emph{`O'} sentences were observed during training. Moreover, applying the pretrained $BILSTM_{cls}^{bert}$ to the \emph{debate.org} data set yields very low precision and recall on \emph{`B'} sentences. In contrast to the \emph{Student Essay} data set where arguments often begin with cue words (e.g., \emph{first}, \emph{second}, \emph{however}), the documents in the \emph{debate.org} data set use cue words less often, impacting the classification performance.


The results from training the $BILSTM_{cls}^{bert}$ model from scratch on the \emph{debate.org} data set are very different to our results on the \emph{Student Essay} data set. As shown in Table \ref{tab:Results:CM}, the confusion matrix for the \emph{debate.org} data set show that the BiLSTM model has difficulties to learn which sentences start an argument in the \emph{debate.org} data set. In contrast to the \emph{Student Essay} data set, it cannot learn from the peculiarities (e.g., cue words) and apparently fails to find other indications for \emph{`B'} sentences. In addition, also the distinction between \emph{`I'} and \emph{`O'} sentences is not clear. These results match our experiences with the annotation of documents in the \emph{debate.org} data set where it was often difficult to decide whether a sentence form an argument and to which argument it belongs. This is also reflected by the inter-annotator agreement of 0.24 based on Krippendorff's $\alpha$ on a subset of 20 documents with three annotators.

Overall, we find that the performance of the argument identification strongly depends on the peculiarities and quality of the underlying data set. For well curated data sets such as the \emph{Student Essay} data set, the information contained in the current sentence as well as the surrounding sentences yield an accurate identification of arguments. In contrast, data sets with poor structure or colloquial language, as given in the \emph{debate.org} data set, lead to less accurate results.%task harder as reflected by our results.


%***********************ARGUMENT CLUSTERING***************************

\subsubsection{Argument Clustering}
\label{sec:Results:AS}


In the final step of the argument search framework, we evaluate the argument clustering according to topical aspects based on the \emph{debatepedia} data set. Therefore, we evaluate the performance of the clustering algorithms HDBSCAN and k-means for different document embeddings that yielded the best results in the topic clustering step of our framework. We estimate the parameter $k$ for the k-means algorithm for each topic using a linear regression based on the number of clusters relative to the number of arguments in this topic. As shown in Figure \ref{fig:Results:Correlation}, we observe a linear relationship between the number of topical aspects and the argument count per topic in the \emph{debatepedia} data set. As shown in Table \ref{tab:Results:ASUnsupervised}, we perform the clustering based on the arguments in each ground-truth topic separately and average the results across the topics. We observe that HDBSCAN performs best on tf-idf embeddings with an averaged $ARI$ score of 0.085 while k-means achieves its best performance on \emph{bert-avg} embeddings with an averaged $ARI$ score of 0.065. Using HDBSCAN instead of k-means on tf-idf embeddings yields an improvement in the $ARI$ score of 2.7\%. Using k-means instead of HDBSCAN on \emph{bert-avg} and  \emph{bert-cls} embeddings results in an improvement of 4.7\% and 2.8\%, respectively. 


Using an UMAP dimensionality reduction step before applying HDBSCAN outperforms k-means on \emph{bert-avg} embeddings with an $ARI$ score of 0.069. However, on tf-idf embeddings using an UMAP dimensionality reduction step slightly reduces the performance. Comparing the results of using \emph{bert-cls} embeddings versus \emph{bert-avg} embeddings, we find that \emph{bert-avg} embeddings result in slightly better scores with a maximum improvement of 2.1\%. We further compare calculating tf-idf vectors only within each topic relative to computing them based on all arguments in the whole dataset (\emph{across topics}). This change only affects the document frequencies used to calculate the tf-idf scores. Therefore, terms that are characteristic for a given topic are likely to show higher document frequencies and thus lower tf-idf scores when the computation is performed within each topic. Since tf-idf scores indicate the relevance of each term, clustering algorithms focus more on terms which distinguish the arguments from each other within a topic.
%Hence, characteristic terms which are shared by most arguments in that topic.
Accordingly, the observed deviation of the $ARI$ score by 0.9\% for k-means and 6.1\% for HDBSCAN in combination with UMAP matches our expectation. 
%Finally, the results of the best HDBSCAN model are shown in Table \ref{tab:Results:ASUnsupervised}.
We also evaluated the exclusion of the HDBSCAN noise clusters (\emph{without noise}) yielding an $ARI$ score of 0.140 and a $BCubed~F_1$ score of 0.439.


Furthermore, we show in Table \ref{tab:Results:BestTopics} for the best performing k-means and HDBSCAN models the topics with the highest $ARI$ scores. We observe that the clustering performance on topics with the best clustering performance is still relative low, in particular when compared to the results of the topic clustering step. As indicated by decreasing $ARI$ scores, both models have only a few topics where they perform comparatively well. 

Figure~\ref{fig:Results:Scatterplot} shows the performance of the two models with respect to the number of arguments in each topic. Both $ARI$ and $BCubed~F_1$ scores show a very similar distribution for topics with different numbers of arguments, while the distributions of the homogeneity score show a slight difference for the two models. This indicates that the performance of the clustering algorithms does not depend on the number of arguments. 
%
Moreover, the upper histogram in Figure \ref{fig:Results:Hist} displays the distribution of the degree of consensus between the two models based on the $ARI$ scores for each topic. Comparing this with the distribution of the $ARI$ score computed between the HDBSCAN model and the ground-truth displayed on the histogram below, we observe that the consensus between the two models is, for most topics, rather low.
%. and as such comparable to the agreement with the ground-truth clustering. 

Overall, our results show the difficulties of argument clustering based on topical aspects. %Considering  both the number of arguments and ground-truth clusters within a topic
Based on the \emph{debatepedia} data set, we show that unsupervised clustering algorithm with the proposed embedding methods cannot cluster arguments into topical aspects in a consistent and reasonable way. This result is in line with the results of Reimers et al.~\cite{Reimers2019} stating that even experts have difficulties to identify argument similarity based on topical aspects.
%and consequently they report a low agreement for annotating argument pairs.
Considering that their evaluation is based on sentence-level arguments, it seems likely that assessing argument similarity is even harder for arguments comprised of one or multiple sentences.
Moreover, the authors report promising results for the pairwise assessment of argument similarity when using the output corresponding to the BERT $[CLS]$ token. 
%We applied their approach to the arguments in the \emph{debatepedia} data set but can not confirm their results on this data set (not shown).
However, our experiments show that their findings do not apply to \emph{debatepedia} data set. We assume that this is due to differences in argument similarity that are introduced by using prevalent topics in the \emph{debatepedia} data set rather than using explicitly annotated arguments.
%in the case of Reimers et al. \cite{Reimers2019}.


%In conclusion, our results show the difficulty of the argument clustering. Regardless of the number of arguments and ground-truth clusters within a topic, the selected word embedding and clustering algorithm, we find no successful method to cluster arguments into topical aspects for the \emph{debatepedia} data set. This result is in line with the results of Reimers et al. \cite{Reimers2019} who point out how difficult it is even for experts to identify argument similarity based on topical aspects and consequently they report a low agreement for annotating argument pairs. Considering that their evaluation is based on sentential arguments, it seems likely that assessing argument similarity is even harder for arguments comprised of one or multiple sentences. Reimers et al.~\cite{Reimers2019} report promising results for the pairwise assessment of sentential argument similarity when using the output corresponding to the BERT $[CLS]$ token. 
%We applied their approach to the arguments in the \emph{debatepedia} data set but can not confirm their results on this data set (not shown).
%However, our experiments show that their findings do not apply to our data sets. We hypothesize that is due to differences in argument similarity induced by using subtopics in debatepedia.org relative to using explicitly annotated arguments in the case of Reimers et al. \cite{Reimers2019}.

\fi 
